When in Doubt: Neural Non-Parametric Uncertainty Quantification for Epidemic Forecasting

Accurate and trustworthy epidemic forecasting is an important problem that has impact on public health planning and disease mitigation. Most existing epidemic forecasting models disregard uncertainty quantification, resulting in mis-calibrated predictions. Recent works in deep neural models for uncertainty-aware time-series forecasting also have several limitations; e.g. it is difficult to specify meaningful priors in Bayesian NNs, while methods like deep ensembling are computationally expensive in practice. In this paper, we fill this important gap. We model the forecasting task as a probabilistic generative process and propose a functional neural process model called EPIFNP, which directly models the probability density of the forecast value. EPIFNP leverages a dynamic stochastic correlation graph to model the correlations between sequences in a non-parametric way, and designs different stochastic latent variables to capture functional uncertainty from different perspectives. Our extensive experiments in a real-time flu forecasting setting show that EPIFNP significantly outperforms previous state-of-the-art models in both accuracy and calibration metrics, up to 2.5x in accuracy and 2.4x in calibration. Additionally, due to properties of its generative process,EPIFNP learns the relations between the current season and similar patterns of historical seasons,enabling interpretable forecasts. Beyond epidemic forecasting, the EPIFNP can be of independent interest for advancing principled uncertainty quantification in deep sequential models for predictive analytics

==> checklist.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{We mention the setup for training and inference in Section 3 and 5. Details on hyperparameters are provided in Supplementary.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{See Section \ref{sec:mainres}}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See Section \ref{sec:experiments}}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{All data we use is anonymized, publicly accessible and distributed by CDC}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> dump.tex <==
\begin{table}
% \vspace{-10pt}
\centering
\caption{Baselines: upper are flu forecasting related; lower are general ML uncertainty related.}
\scalebox{0.9}{\small
\begin{tabular}{p{0.3\textwidth} p{0.64\textwidth}}
\toprule
Baseline model                          & Description                                                                                                                                                                      \\ \midrule
SARIMA                         & Seasonal ARIMA, time series model used in \cite{adhikari_epideep_2019, zimmer_influenza_2020}.                             \\
Gated Recurrent Unit (GRU)     &   A popular deep learning sequence encoder.                                                                                                          \\
Empirical Bayes (EB)           & Bayes framework. Won a few epidemic forecasting competitions~\cite{brooks_flexible_2015}.                                                                                   \\ 
Delta Density (DD)             & A former top performing method \cite{reich_collaborative_2019}. Learns distribution of change in successive wILI values~\cite{brooks_nonmechanistic_2018}. \\
EpiDeep (ED)                   & Recent NN flu model based on learning similarity between seasons~\cite{adhikari_epideep_2019}.                                                       \\
Gaussian Process (GP)          & Recently proposed statistical flu prediction model \cite{zimmer_influenza_2020}.                                                                                                  \\ \midrule\midrule
Monte Carlo Dropout (MCDP)     & Applies dropout at test time to measure the uncertainty \cite{gal_dropout_2016} (w/ GRU).                              \\
Bayesian neural network (BNN)  & Learns probability distributions over model parameters~\cite{blundell2015weight} (w/ LSTM).                                                           \\
Recurrent Neural Process (RNP) & Builds on Neural Process framework to learn from sequential data \cite{qin_recurrent_2019}.                                                                           \\ \bottomrule
% \end{tabular}
\end{tabular}
}
\vspace{-10pt}
\label{tab:baselines}
\end{table}


\begin{wraptable}[19]{r}{.56\linewidth}
\vspace{-8pt}
\centering
\caption{Evaluation metrics\label{tab:metrics}}
\vspace{-2pt}
\scalebox{0.9}{\small
    \begin{tabular}{p{0.2\textwidth} p{0.38\textwidth}}
\toprule
Model                          & Description                                                                                                                                                                      \\ \midrule
Root~Mean~Sq.~Error                         & $RMSE(M)=$ $\sqrt{\frac{1}{T}\sum_{t=1}^{T}(y_{N+1}^{(t)} - \hat{y}_{N+1,M}^{(t)})^2}$                          \\ \midrule
Mean~Abs.~Per.~Error    &   $MAPE(M) = \frac{1}{T}\sum_{t=1}^T \frac{|y_{N+1}^{(t)} - \hat{y}_{N+1,M}^{(t)}|}{|y_{N+1}^{(t)}|}$                                                                                             \\ \midrule
Log Score (LS): Probabilistic metric used by the CDC~\cite{reich_collaborative_2019}.           & $LS(M)=$ $\sum_{i=1}^T \frac{1}{T}\int_{y_{i}^{( t)} - 0.5}^{y_{i}^{(t)} + 0.5} - \log (\hat{p}_{N+1,M}^{(t)}(y))dy$     \\ \midrule
Calibration Score (CS): our metric  inspired from reliability diagrams for binary events \cite{niculescu-mizil_predicting_2005} to favor \emph{well calibrated models that provide meaningful confidence intervals} & 
Define function $k_M: [0,1] \rightarrow [0,1]$ for model $M$ as follows. For each  confidence value $c \in[0,1]$, let $k_M(c)$ denote the fraction of observed ground truth that lies inside the $c$ confidence interval of predicted output distributions of $M$.
Thus, for a perfectly calibrated model $M^*$ we would expect $k_{M^*}(c)=c$. CS measures the deviation of $k_{M}$ from $k_{M^*}$: $CS(M)=\int_{0}^1 |k_M(c)-c| dc \approx 0.01 \sum_{c\in\{0, 0.01, \dots, 1\}} |k_M(c)-c|$
\\ \bottomrule
% \end{tabular}
\end{tabular}%\vspace{-2in}
}
\end{wraptable}


==> related.tex <==
\section{Additional Related work}
For more details, please refer to the Appendix.
% \zc{too short, write at least 0.5 pages}

\noindent
\textbf{Statistical Models for Epidemic Forecasting}:
Statistical models alluded to in Section \ref{sec:intro} include models designed to model the details on the underlying generative distribution such as: Empirical Bayes framework \cite{brooks_flexible_2015} that constructs a prior of the current season's epidemic curve from  past seasons and outputs a distribution over epidemic curves; Kernel Density estimation \cite{brooks_nonmechanistic_2018} that models the probability distribution of the change between consecutive predictions; and Gaussian processes~\cite{zimmer_influenza_2020}. Other popular methods rely on ensembles of mechanistic and statistical methods ~\cite{ray2020ensemble}. 
% \zc{descriptions for these methods are too simple, need some technical summarization to highlight their major ideas and assumptios}% check later last citation, which may not be accurate

More recently, deep learning models have been crafted for forecasting influenza \cite{adhikari_epideep_2019, wang2019defsi} and COVID-19 \cite{rodriguez_deepcovid_2021, qian2020and}, whose expressive power enable addressing novel situations such as %traditional flu models fail such as adapting a historical influenza model to pandemic
adapting a historical flu model to the pandemic via transfer learning
\cite{rodriguez_steering_2020}. 
%Deep learning is also suitable because it provides the capability of ingesting data from multiple sources. 
However, as mentioned before, uncertainty quantification is often neglected or done using relatively simpler methods. %Our work aims to close this gap in the literature. 
% \zc{need to comment on their limitations, and/or justify their differences from ours}

\noindent\textbf{Uncertainty Quantification for Deep Learning}: %Recent works have shown that deep neural networks are over-confident in their predictions \cite{guo2017calibration, kong2020calibrated}.
%Existing approaches for uncertainty quantification  can be categorized into two lines. The first line is based on 
Bayesian Neural Networks (BNNs) \cite{mackay1992practical, blundell2015weight, louizos2017multiplicative} are realized by first imposing prior distributions over NN parameters, next inferring parameter posteriors
and integrating over them to make predictions. However, due to intractability of posterior inference,
approximation methods have also been proposed, including variational inference \cite{blundell2015weight, louizos2017multiplicative}, Monte
Carlo dropout \cite{gal_dropout_2016} and stochastic gradient Markov chain Monte Carlo (SG-MCMC) \cite{li2016preconditioned, Zhang2020Cyclical}.
Apart from the problem of specifying reasonable parameter priors for BNNs with large number of parameters, they also underestimate the uncertainty \cite{kong2020sde}.

%\noindent\textbf{Neural Process}:

Neural Process (NP), a recently introduced framework
\cite{garnelo_neural_2018} attempts to combine the stochastic processes and DNNs. It  defines a distribution over a global latent variable to capture the functional uncertainty, while Functional Neural Process (FNP) \cite{louizos_functional_2019}  uses a dependency graph to encode the data correlation uncertainty. However, they are both for the static data. Recently, Recurrent Neural Process (RNP) \cite{qin_recurrent_2019} has been proposed to incorporate RNNs into the NP to capture the sequential information. 
Our method, however, has stronger representation power and more explainable predictions (see Section \ref{sec:method}).
%Deep ensemble \cite{lakshminarayanan2017simple}  which train multiple DNNs suffer from requirement of extensive computing resources.

